Reactivity of Ambident Nucleophiles in Magnetic Fields: a Combined Conceptual DFT and Current-DFT Study

The influence of strong external magnetic fields (up to $0.30\,B_0$) on the electronic structure and reactivity of ambident nucleophiles is investigated using the nitrite and thiocyanate anions as prototypical examples. To capture magnetic-field-induced changes in reactivity, current-density-functional theory (current-DFT) calculations are interpreted through conceptual density-functional theory (conceptual DFT) descriptors, namely global hardness and local softness via Fukui functions, focusing on the evolution of the electronic structure and associated properties with increasing field strength in different orientations. By extending our previous adiabatic treatment of molecules to include higher-spin states, in analogy with earlier work on atoms, and by considering the symmetry properties of relevant quantum-chemical quantities within full magnetic groups using the QSym$^2$ framework, we uncover substantial magnetic-field-induced modulations of both molecular polarity and the shape of the Fukui function. Despite these modulations, the ambident nucleophilicity of both $(\textrm{NO}_2)^-$ and $\textrm{SCN}^-$ is largely preserved, as is the preference for attack by soft electrophiles at the sulfur end of $\textrm{SCN}^-$. At higher field strengths, however, the Fukui functions become increasingly diffuse, reflecting the growing importance of external magnetic interactions relative to internal electrostatic forces. The resulting redistribution of local reactivity not only predicts reaction pathways with unexpected geometries but also raises the possibility that regioselectivity may become progressively less well-defined in the strong-field regime.

==> suppinfo/preamble.tex <==
% ========
% Preamble
% ========



% ------------------
% Scientific support
% ------------------
% Chemistry
\usepackage[version=4]{mhchem}

% Scientific typesetting
\usepackage{siunitx}
\DeclareSIUnit{\atomicunit}{a.u.}
\DeclareSIUnit{\atomicmassunit}{u}
\DeclareSIUnit{\angstrom}{\text {Å}}
\DeclareSIUnit{\cal}{cal}

% -------------
% Maths support
% -------------
\usepackage{%
  amsthm,%
  amssymb,%
  mathrsfs,%
  mathtools,%
  gensymb,%
  braket,%
  mleftright,%
  nicefrac,%
  interval%
}
\intervalconfig{%
  soft open fences%
}

\mleftright

\newcommand*\bmmax{2}
\usepackage{bm}


% --------
% Diagrams
% --------

% Colours
\usepackage[usenames, svgnames, x11names, rgb]{xcolor}

% Graphics
\usepackage{graphicx}

% --------
% Captions
% --------
\usepackage{caption, subcaption}


% ------
% Tables
% ------
\usepackage{%
  booktabs,%
  array,%
  adjustbox,%
  makecell,%
  multirow,%
  bigdelim%
}
\newcolumntype{M}[1]{>{\centering\arraybackslash}m{#1}}
\newcolumntype{L}[1]{>{\raggedright\arraybackslash}m{#1}}
\newcolumntype{R}[1]{>{\raggedleft\arraybackslash}m{#1}}

% -----
% Items
% -----
\usepackage[inline]{enumitem}


% ----------
% Hyperlinks
% ----------
\usepackage[%
  hyperfootnotes=false,%
  hypertexnames=false,%
  hidelinks,%
]{hyperref}
\hypersetup{%
  bookmarksnumbered=true,%
  colorlinks=true,%
  citecolor=teal,%
  linkcolor=Blue4,%
}


% ------------
% Bibliography
% ------------
\usepackage{mciteplus}

% ---------
% Debugging
% ---------
%\listfiles
